Leveraging Transitive Relations for Crowdsourced Joins

The development of crowdsourced query processing systems has recently attracted a significant attention in the database community. A variety of crowdsourced queries have been investigated. In this paper, we focus on the crowdsourced join query which aims to utilize humans to find all pairs of matching objects from two collections. As a human-only solution is expensive, we adopt a hybrid human-machine approach which first uses machines to generate a candidate set of matching pairs, and then asks humans to label the pairs in the candidate set as either matching or non-matching. Given the candidate pairs, existing approaches will publish all pairs for verification to a crowdsourcing platform. However, they neglect the fact that the pairs satisfy transitive relations. As an example, if $o_1$ matches with $o_2$, and $o_2$ matches with $o_3$, then we can deduce that $o_1$ matches with $o_3$ without needing to crowdsource $(o_1, o_3)$. To this end, we study how to leverage transitive relations for crowdsourced joins. We propose a hybrid transitive-relations and crowdsourcing labeling framework which aims to crowdsource the minimum number of pairs to label all the candidate pairs. We prove the optimal labeling order in an ideal setting and propose a heuristic labeling order in practice. We devise a parallel labeling algorithm to efficiently crowdsource the pairs following the order. We evaluate our approaches in both simulated environment and a real crowdsourcing platform. Experimental results show that our approaches with transitive relations can save much more money and time than existing methods, with a little loss in the result quality.

==> crowdsource-label-algo.tex <==

%% $Id$
\begin{figure}[htup]
\begin{algorithm}[H]

\linesnumbered \SetVline

\small
\caption{\textsc{CrowdsourceLabel}($p$)}

\SetLine

\KwIn{$p$~: an object pair}
 \KwOut{$\ell$: the crowdsourced label}

\SetVline
%\max_{\theta\in\Theta}\theta

\Begin{
    HIT = \textsf{CreateHIT}($p$)\;
    \textsf{PublishHIT}(HIT)\;
    $\ell$ = \textsf{WaitForCrowdsourcedLabel}()\;
    \textbf{return} $\ell$\;
}
\end{algorithm} \vspace{-1em}
\caption{An algorithm for crowdsourcing the label of an object pair.}\label{algo:crowdsource-label}
\end{figure} 

==> label-overview-algo.tex <==

%% $Id$
\begin{figure}[tup]
\begin{algorithm}[H]

\linesnumbered \SetVline

\small
\caption{\textsc{Labeling}($\order$)}

\SetLine

\KwIn{$\order = \langle p_1, p_2, \cdots, p_n \rangle$~: a sorted list of unlabeled pairs}
 \KwOut{$\labelset = \{(p_i, \ell)~|~1 \leq i\leq n\}$: a set of labeled pairs}

\SetVline
%\max_{\theta\in\Theta}\theta

\Begin{

    $\labelset = \{\}$\;
    \For {\emph{$i=1$ to $n$}}{
       $\ell$ = \textsf{DeduceLabel}($p_i$, $\labelset$)\;
       \If { \emph{$\ell$ = ``undeduced"} }{
            $\ell$ = \textsf{CrowdsourceLabel}($p_i$)\;
        }
        Add $(p_i, \ell)$ into $\labelset$\;
    }
    \textbf{return} $\labelset$\;

}
\end{algorithm} \vspace{-1em}
\caption{Labeling algorithm.}\label{algo:labeling-overview}\vspace{-1em}
\end{figure}


==> label.tex <==

\section{Labeling}\label{sec:simple-labeling}
Given a set of object pairs, after identifying their best labeling order, i.e. the expected optimal labeling order, we need to consider how to label them in the identified order. In this section, we first present the overview of our labeling algorithm in Section~\ref{subsec:overview}. The algorithm mainly consists of two important parts, deducing the label of an object pair and crowdsourcing the label of an object pair. We respectively discuss their efficient implementations in Section~\ref{subsec:label-deduction} and~\ref{subsec:label-crowdsourcing}.


%As we need to label the given set of pairs in a specific order, we need to start with the first pair in the order, and label each pair one after another.

\subsection{Labeling Algorithm}\label{subsec:overview}
Figure~\ref{algo:labeling-overview} shows the overview of our labeling algorithm. Given a labeling order $\order = \langle p_1, p_2, \cdots, p_n\rangle$, the algorithm will first label the first pair $p_1$, and then the second pair $p_2$, the third pair $p_3$, etc. When labeling the $i$-th pair $p_i$, if its label cannot be deduced from the already labeled pairs, i.e., $\{p_1, p_2, \cdots, p_{i-1}\}$, we publish $p_i$ to a crowdsourcing platform and wait for its crowdsourced label; otherwise, we output its deduced label. After obtaining the label of $p_i$, we begin to process the next pair $p_{i+1}$, and use the same method to get its label. The algorithm stops until all the pairs are labeled.
\input{label-overview-algo}

\subsection{Deducing the label of an object pair}\label{subsec:label-deduction}
A key problem of our approach is how to decide whether a pair $p = (o, o')$ can be deduced from the already labeled pairs $\labelset$. As mentioned in Section~\ref{sec:system-framework}, we need to check whether there is a path from $o$ to $o'$ in the graph built for $\labelset$ which contains no more than one non-matching pair. One naive solution is to enumerate every path between $o$ and $o'$, and check the number of non-matching pairs in each path. This solution is very expensive since the number of the paths increases exponentially with the number of objects in the graph. In the following, we propose a graph-clustering-based method to solve this problem.




\input{deduce-label-algo}

Recall that to decide whether a pair can be deduced from $\labelset$, we only need to count the number of non-matching pairs in each path from $o$ to $o'$, whereas the number of matching pairs is not important for the decision. This observation inspires us to merge the matching objects into the same cluster, and then add the ``non-matching" labeled edges among different clusters. We call such graph \clustergraph. By using the \clustergraph, we can efficiently decide whether a new pair $p=(o, o')$ can be deduced from the already labeled pairs. Figure~\ref{algo:deduce-label} shows the pseudo-code of the algorithm. Given a set of labeled pairs $\labelset$, we first build a \clustergraph for $\labelset$ (Line~\ref{algo:deduce-label:buildgraph}). Then for the unlabeled pair $p=(o, o')$, (1) if $o$ and $o'$ in the same cluster, then there is a path from $o$ to $o'$ which only consists of matching pairs, thus $o$ and $o'$ can be deduced as a matching pair (Lines~\ref{algo:deduce-label:matching-begin}-\ref{algo:deduce-label:matching-end}); (2)if $o$ and $o'$ in different clusters but there is an edge between them, then there exists a path from $o$ to $o'$ which contains a single non-matching pair, thus $o$ and $o'$ can be deduced as a non-matching pair (Lines~\ref{algo:deduce-label:nonmatching-begin}-\ref{algo:deduce-label:nonmatching-end}); If $o$ and $o'$ in different clusters and there is no edge between them, then there does not exist a path from $o$ to $o'$ which contains no more than one non-matching pair, thus $o$ and $o'$ cannot be deduced (Lines~\ref{algo:deduce-label:undeduced-begin}-\ref{algo:deduce-label:undeduced-end}).

\begin{figure}[htbp]
\centering
  \includegraphics[scale=0.35]{figs/cluster-graph.eps}\\
  \caption{A {$\clustergraph$} built for the first seven labeled pairs $\{p_1, p_2, \cdots, p_7\}$ in Figure~\ref{fig:framework}.}\label{fig:cluster-graph}
\end{figure}


\begin{example}
Suppose we have already labeled the first seven pairs $\{ p_1, p_2, \cdots, p_7\}$ in Figure~\ref{fig:deduce-graph}. To decide whether $p_8$ can be deduced from the already labeled pairs, we build a $\clustergraph$ as shown in Figure~\ref{fig:cluster-graph}. As $o_1, o_2, o_3$ are matching, we merge them into one cluster. As $o_4$ and $o_5$ are matching, we merge them into another cluster. Since $o_6$ does not match with any other object, we take itself as one cluster. After clustering all the matching objects in the $\clustergraph$, we obtain three clusters. In the already labeled pairs $\{ p_1, p_2, \cdots, p_7\}$, there are three non-matching pairs, i.e., $p_3=(o_1, o_6)$, $p_6=(o_4, o_6)$, $p_7=(o_2, o_4)$. We respectively add three non-matching edges between $\cluster{o_1}$ and $\cluster{o_6}$, $\cluster{o_4}$ and $\cluster{o_6}$, $\cluster{o_2}$ and $\cluster{o_4}$ to the $\clustergraph$.  For the unlabeled pair $p_8=(o_5, o_6)$, since $o_5$ and $o_6$ are in different clusters, and $\cluster{o_5}$ and $\cluster{o_6}$ have an edge in the \clustergraph, then there must exist a path from $o_5$ to $o_7$ which contains a single non-matching pair (i.e., $o_5\!\rightarrow\!o_4\!\rightarrow\!o_6$), thus $p_8=(o_5, o_6)$ can be deduced as a non-matching pair from the already labeled pairs $\{p_1, p_2, \cdots, p_7\}$.
\end{example}

%can be deduced as a matching pair since they are in the same cluster, and $(o_5, o_7)$ can be deduced as a non-matching pair since they are in different clusters and $\cluster{o_5}$ and $\cluster{o_7}$ have an edge, and $(o_1,o_7)$ cannot be deduced since they are in different clusters and $\cluster{o_1}$ and $\cluster{o_7}$ have no edge.




\iffalse
To build \clustergraph, initially, each object itself is taken as a cluster, and there is no edge among the clusters. Let $\cluster{o}$ denote $o$'s cluster. When adding a new pair $(o, o')$ to the graph, we consider the following cases: (1) If $o$ and $o'$ are in the same cluster, i.e. $\cluster{o} = \cluster{o'}$, the graph will keep unchanged; (2) If $o$ and $o'$ are in the different clusters, i.e. $\cluster{o} \neq \cluster{o'}$, and $o$ and $o'$ are non-matching, we will add an edge (if not exists) labeled ``non-matching" between \cluster{o} and \cluster{o'} to the graph; (3) If $o$ and $o'$ are in the different clusters, i.e. $\cluster{o} \neq \cluster{o'}$, and $o$ and $o'$ are matching, we will merge the objects in $\cluster{o}$ and $\cluster{o'}$ into a new cluster, and for each cluster that originally has an edge with $\cluster{o}$ or $\cluster{o'}$, we remove the edge from the graph, and then add a new edge with the merged cluster. For example, suppose  . To build .


\fi





\subsection{Crowdsourcing the label of an object pair}\label{subsec:label-crowdsourcing}
If a pair's label cannot be deduced from the already labeled pairs, we will create a Human Intelligent Task (HIT) for the pair, and publish it to a crowdsourcing platform. Figure~\ref{fig:hit-example} shows an example HIT for a pair (``\textsf{iPad 2}", ``\textsf{iPad two}"). In the HIT, there is a pair of strings, ``\textsf{iPad 2}" and ``\textsf{iPad two}", and the workers are required either select ``YES" if they think ``\textsf{iPad 2}" and ``\textsf{iPad two}" are mathing, or select ``NO" if they think ``\textsf{iPad 2}" and ``\textsf{iPad two}" are not matching, and then they submit their answers by clicking the \textsf{SUBMIT} button. After the crowd workers complete the HIT, we output the crowdsourced label of the pair.

\begin{figure}[htbp]
\centering
  \includegraphics[scale=0.3]{figs/hit.eps}\\
  \caption{An example HIT for an object pair.}\label{fig:hit-example}
\end{figure}

%\input{crowdsource-label-algo}







==> misc.tex <==
 %affect the crowdsourced joins. exist for crowdsourced joins, such as one-to-one and many-to-one relations.  For example, one-to-one relation means that an object from one collection

%; (2) for the dataset with not so many matching objects, transitive relations can help to save some money with a little bit of loss in result quality but may lead to longer completion time.











(1) our approaches with transitive relations can save much more money and time than existing methods, with a little loss in the result quality.

There are many future directions



The experimental results on a real dataset show that there are about 26 times difference between the best and the worst labeling orders.



 the drawbacks of , and . To address this problem. we devised a parallel labeling



 was presented.


 which lead to the minimum expected number of crowdsourced pairs. We devised a parallel-labeling .

have shown that transitive relations can save the number of crowdsourced pairs that need to be crowdsourced by more than 20 times.

using transitive relations to crowdsource the minimum number of pairs to label a set of pairs. We propose

We formulate the problem of leveraging transitive relations

1. transitive relations effect
2. order significant effect
3. expected order
4. parallel labeling
5. real crowdsourced result


Future work
1. other rules in crowdsourced joins. one-to-one mapping
2. other rules in crowdsourced query, for sorting
3. Ambiguity,
4. More flexible tradeoffs.



uk



that whether there is a path from $o$ to $o'$ which contains no more than one non-matching pair.



Based on this idea, we study which pairs can be crowdsourced together for a given sorted list of object pairs. We know that a pair $p_i = (o, o')$ needs to be crowdsourced if an only if $p_i$ cannot be deduced from $\{p_1, p_2, \cdots, p_{i-1}\}$. In the case that the labels of $p_1, p_2, \cdots, p_{i-1}$ are known, we only need to check the graph built for $\{ p_1, p_2, \cdots, p_{i-1}\}$ that whether there is a path from $o$ to $o'$ which contains no more than one non-matching pair. However, before crowdsourcing any pair, the labels of $\{p_1, p_2, \cdots, p_{i-1}\}$ are unknown. In this case, we check the graph built for $p_1, p_2, \cdots, p_{i-1}$ whether there exists a path from $o$ to $o'$. This is because if such path does not exist, then there is no path from $o$ to $o'$ which contains no more than one non-matching pair, thus $p_i$ must need to be crowdsourced. For example, consider the labeling order $\order = \{(o_1, o_2), (o_2, o_3), (o_3, o_4)\}$. For the third pair $(o_3, o_4)$, since there is no path from $o_3$ to $o_4$ in the graph built for the first two pairs, $(o_3, o_4)$  must not be deduced from $(o_1, o_2)$ and $(o_2, o_3)$, thus it needs to be crowdsourced.


Given a sorted list of object pairs $\order$, by using the above method, we can select a set of pairs which must need to be crowdsourced, and then publish them to the crowdsourced platform together. When all the published pairs have been labeled by the crowd workers, we need to decide which pairs can be published next. Different from the case that all the pairs are unlabeled, in this case, some pairs are labeled and the others are unlabeled. We first use the existing labeled pairs to deduce the other unlabeled pairs. For the remaining unlabeled pairs, we investigate in which condition they could be published. Consider a unlabel pair $p_i = (o, o')$. We know that if the condition ``\emph{in the graph built for $\{p_1, p_2, \cdots, p_{i-1}\}$, for each path from $o$ to $o'$, the number of non-matching pairs in the path is larger than one}" holds, then $p_i$ cannot be deduced from $\{ p_1, p_2, \cdots, p_{i-1}\}$, thus it will be published. However, there may be some pairs in $\{p_1, p_2, \cdots, p_{i-1}\}$ whose labels are unknown. To ensure the condition holds for any possible labels, we assume all the unlabeled pairs are matching pairs. If the condition holds for this case, it holds no matter which labels the unlabeled pairs are.


we can publish $p_i$,




We need to select from the unlabeled pairs that must need to be crowdsourced.


we can use them to deduce some of the other published pairs.

we need to decide which pairs can be published next. We first use the existing crowdsourced pairs to deduce some unpublished pairs in $\order$. Let $\labelset$ denote the labeled pairs. After doing that, the pair in $\order$ has three different types of labels,


 and wait for their crowdsourced labels.


For example, .





However, when

there is no path from $o_1$ to $o_2$ in


Based on this idea, we


 all need to publish the can publish it

If we first publish $(o_1, o_2)$

For a pair



%Based on this idea, we propose a novel framework to label a given set of object pairs through crowdsourcing and transitivity.


%However, some of the object pairs is not necessary to be checked by the crowd as their labels can be deduced according to transitivity property. Based on this idea, we propose a novel framework to label them. The framework iteratively interacts with the crowdsourcing platform by first identifying some object pairs that need to be published, and then using the transitivity to deduce the labels of some other object pairs based on the labels of existing published object pairs.

\label{subsec:transitivity}
%\reminder{transitivity may not always hold.}
\begin{definition}[Positive Transitivity]\label{def:positive-transitivity}
Given three objects, $o_1$, $o_2$ and $o_3$, if $o_1=o_2$, and $o_2=o_3$, then we have $o_1=o_3$.
\end{definition}

For example, consider three strings ``\textsf{ipad 2}", ``\textsf{ipad 2nd}" and ``\textsf{ipad two}". As ``\textsf{ipad 2}" and ``\textsf{ipad 2nd}" are matching, ``\textsf{ipad 2nd}" and ``\textsf{ipad two}" are matching, then ``\textsf{ipad 2}" and ``\textsf{ipad two}" must be matching.




%Typically, we need to pay the crowd workers some money for labeling object pairs, so the fewer number of crowdsourced pairs leads to less money.


\begin{theorem}

\end{theorem}

lemma 2 general negative transitivity

theorem 1, deduce and crowdsource

define crowdsourced pair/deduced pair







%then we only need to crowdsource the first two pairs


%first label $(o_i, o_k)$ and $(o_k, o_j)$, the crowd will return $o_i=o_k$ and $o_k\neq o_j$.\footnote{In our paper, we assume that the crowd always returns correct answers. Although this is not true in reality, there is a lot of existing work to solve this problem~\cite{Ipeirotis2010, journals/pvldb/LiuLOSWZ12} which is orthogonal to our problem.} Then we can avoid publishing $(o_i, o_j)$ as $o_i\neq o_j$ can be deduced based on Definition~\ref{def:negative-transitivity}. Therefore, in this order, we need to publish \emph{two} object pairs in total. However, if we first publish $(o_k, o_j)$ and $(o_i, o_j)$, the crowd will return $o_k \neq o_j$ and $o_i\neq o_j$. We still have no idea about the label of $(o_i, o_j)$ from the results, thus need to publish $(o_i, o_j)$ as well. Therefore, in this order, we need to publish \emph{three} object pairs in total. Typically, we need to pay the workers for labeling object pairs, so the fewer number of published pairs leads to less money. In order to spend the least money, our framework first seeks to find the optimal order to publish object pairs, and then label the pairs in this order. Figure~\ref{fig:framework} shows our framework. Specifically, the framework consists of two steps.




%Our framework labels a set of object pairs through crowdsourcing and transitivity.




%based on Lemma~\ref{lem:transitivity}


%Given a set of unlabeled object pairs, in order to utilize transitivity to deduce their labels, we have to first publish some object pairs to the crowdsourcing platform, and then deduce the labels of other object pairs based on the labels of published object pairs.


\begin{theorem}
Given a set of labeled object pairs, $\{p_1, p_2, \cdots, p_n\}$,  let $G$ denote the graph build on $\{p_1, p_2, \cdots, p_n\}$. For a new pair $p=(o, o')$, (1) $p$ is deduced as a matching pair iff. there is a path from $o$ to $o'$ which only consists of matching pairs; (2) $p$ is deduced as a non-matching pair iff. there is a path from $o$ to $o'$ which only contains a single non-matching pairs; (3) $p$ cannot be deduced iff. there does not exist any path from $o$ to $o'$ which only consists of matching pairs;
\end{theorem}

\begin{definition}[Negative Transitivity]\label{def:negative-transitivity}
Given three object, $o_1$, $o_2$ and $o_3$, if $o_1=o_2$, and $o_2\neq o_3$, then we have $o_1\neq o_3$.
\end{definition}

For example, consider three strings ``\textsf{ipad 2}", ``\textsf{ipad two}" and ``\textsf{iphone 4}". As ``\textsf{ipad 2}" and ``\textsf{ipad two}" are matching, ``\textsf{ipad two}" and ``\textsf{ipone 4}" are non-matching, then ``\textsf{ipad 2}" and ``\textsf{iphone 4}" must be non-matching.

By applying positive transitivity and negative transitivity for many times, we can easily deduce the following lemma.
\begin{lemma}\label{lem:transitivity}
Given a set of objects, $o_1, o_2, \cdots, o_n$, (1) if $o_i = o_{i+1}$ $(1 \leq i \leq n)$, then we have $o_1 = o_{n+1}$; (2) if $o_i = o_{i+1}$ $(1 \leq i < j)$, $o_j \neq o_{j+1}$ and $o_i = o_{i+1}$ $(j < i \leq n)$, then we have $o_1 \neq o_{n+1}$.
\end{lemma}

Consider an object pair. To decide whether its label can be deduced from existing labeled pairs,
%Next we define negative tansitivity.

\begin{definition}[Crowdsourced and Deduced Pairs]\label{def:crowdsourced-deduced}
Given a labeling order $\order = \langle p_1, p_2, \cdots, p_n \rangle$, we say $p_i$ $(1\leq i \leq n)$ is a crowdsourced pair w.r.t $\order$ if the label of $p_i$ cannot be deduced from $p_1, p_2, \cdots, p_{i-1}$; otherwise, $p_i$ is a deduced pair.
\end{definition}


, if swapping $p_i$ and $p_{i+1}$, we can obtain a new labeling order $\order'=\langle p_1, \cdots, p_{i+1}, p_{i}, \cdots, p_n \rangle$. The next question is in which case the new order $\order'$ will require fewer number of crowdsourced pairs than the original order $\order$, i.e. $\cn(\order')\leq \cn(\order)$.

\fussy

We have an observation that swapping $p_i$ and $p_{i+1}$ only has an effect on $p_i$ and $p_{i+1}$. This is because for the pairs $p_j$ $(j\in[1,i-1]\cup [i+2, n])$ in the original order $\order$, $p_j$ is a crowdsourced pair iff. $p_j$ cannot be deduced from $p_1, \cdots, p_{j-1}$.

1. only affect

2.

Suppose $p_i$ is a non-matching pair and $p_{i+1}$ is a matching pair. That is, $\order$ labels a non-matching pair first, but $\order'$ label a matching pair first. Next we compare their number of crowdsourced pairs.


, denoted by
\[\prob(p_i=\textrm{crowdsourced}~|~p_1, p_2, \cdots, p_{i-1})\].




\sloppy


\begin{definition}[Expected Number of Crowdsourced Pairs]
Given a labeling order $\order = \langle p_1, p_2, \cdots, p_n \rangle$, and each object pair $p_i$ $(1 \leq i \leq n)$ is assigned a probability that they are matching, $\order$'s expected number of crowdsourced pairs, denoted by $\ecn(\order)$, is defined as the sum of the probability that each pair needs to be crowdsourced, i.e.,  $\sum_{i=1}^{n} \prob(p_i~|~p_1, p_2, \cdots, p_{i-1})$, where $\prob(p_i\ \textrm{is crowdsourced})$ denotes the probability that $p_i$ cannot be deduced from $p_1, p_2, \cdots, p_{i-1}$.
\end{definition}

\fussy

then we have


Recall the optimal labeling order in previsous section. we have

explore the expected optimal labeling order. 

==> overview.tex <==

%we consider the problem of acquiring the labels of a set of object pairs through crowdsourcing, where l
\section{Hybrid Transitive-Relations and Crowdsourcing Labeling Framework}
\label{sec:hybrid-workflow}

This section investigates how to combine transitive relations and crowdsourcing to label a given set of pairs. Figure~\ref{fig:workflow} shows our hybrid transitive-relations and crowdsourcing labeling framework. The framework consists of two components, \texttt{Sorting} and \texttt{Labeling}. We will respectively describe the two components in Sections~\ref{subsec:sorting} and~\ref{subsec:labeling}, and illustrate how the whole framework works in Section~\ref{subsec:workflow-example}.

\begin{figure}[htbp]
\centering
  \includegraphics[scale=0.35]{figs/overview-new.eps}\\
  \caption{Hybrid transitive-relations and crowdsourcing labeling framework.}\label{fig:workflow}
\end{figure}


\subsection{Sorting Component}\label{subsec:sorting}

We have an interesting finding that the order of labeling object pairs will affect the total number of pairs need to be crowdsourced. For example, suppose we need to label three object pairs, $(o_1, o_2)$, $(o_2, o_3)$, $(o_1, o_3)$, where $o_1=o_2$ but $o_2 \neq o_3$ and $o_1 \neq o_3$. If the labeling order is $\big\langle (o_1, o_2), (o_2, o_3), (o_1, o_3)\big\rangle$, after crowdsourcing the first two pairs, we obtain $o_1=o_2$ and $o_2 \neq o_3$. Based on Lemma~\ref{lem:transitivity}, we can deduce that $o_1\neq o_3$, thus this order requires to crowdsource \emph{two} object pairs. However, if we use a different labeling order $\big\langle (o_2, o_3), (o_1, o_3), (o_1, o_2)\big\rangle$, after crowdsourcing the first two pairs, we obtain $o_2 \neq o_3$ and $o_1\neq o_3$. We still need to crowdsource the third pair $(o_1, o_2)$ as its label cannot be deduced based on Lemma~\ref{lem:transitivity}, thus the order requires to crowdsource \emph{three} object pairs.

Typically, in a crowdsourcing platform, we need to pay for crowdsourced pairs, thus there is a financial incentive to minimize the number of crowdsourced pairs. Based on this idea, given a set of unlabeled pairs, the sorting component first identify the optimal labeling order which leads to the fewest number of crowdsourced pairs, and then outputs a sorted list of unlabeled pairs based on the order. The details of identifying the optimal labeling order will be presented in Section~\ref{sec:sorting}.

%which will first seek to identify the best labeling order which results in the fewest number of crowdsourced pairs, and then label the object pairs in the identified order through crowdsourcing and transitive relation. Figure~\ref{fig:framework} shows our labeling workflow.



\subsection{Labeling Component}\label{subsec:labeling}

After identifying the optimal labeling order, we need to consider how to label them in the identified order.


In this section, we first present the overview of our labeling algorithm in Section~\ref{subsec:overview}. The algorithm mainly consists of two important parts, deducing the label of an object pair and crowdsourcing the label of an object pair. We respectively discuss their efficient implementations in Section~\ref{subsec:label-deduction} and~\ref{subsec:label-crowdsourcing}.


%As we need to label the given set of pairs in a specific order, we need to start with the first pair in the order, and label each pair one after another.

\subsubsection{Labeling Algorithm}\label{subsubsec:labeling-algorithm}
Figure~\ref{algo:labeling-overview} shows the overview of our labeling algorithm. Given a labeling order $\order = \langle p_1, p_2, \cdots, p_n\rangle$, the algorithm will first label the first pair $p_1$, and then the second pair $p_2$, the third pair $p_3$, etc. When labeling the $i$-th pair $p_i$, if its label cannot be deduced from the already labeled pairs, i.e., $\{p_1, p_2, \cdots, p_{i-1}\}$, we publish $p_i$ to a crowdsourcing platform and wait for its crowdsourced label; otherwise, we output its deduced label. After obtaining the label of $p_i$, we begin to process the next pair $p_{i+1}$, and use the same method to get its label. The algorithm stops until all the pairs are labeled.
\input{label-overview-algo}

\subsubsection{Deducing the label of an object pair}\label{subsubsec:label-deduction}
A key problem of our approach is how to decide whether a pair $p = (o, o')$ can be deduced from the already labeled pairs $\labelset$. As mentioned in Section~\ref{sec:system-framework}, we need to check whether there is a path from $o$ to $o'$ in the graph built for $\labelset$ which contains no more than one non-matching pair. One naive solution is to enumerate every path between $o$ and $o'$, and check the number of non-matching pairs in each path. This solution is very expensive since the number of the paths increases exponentially with the number of objects in the graph. In the following, we propose a graph-clustering-based method to solve this problem.




\input{deduce-label-algo}

Recall that to decide whether a pair can be deduced from $\labelset$, we only need to count the number of non-matching pairs in each path from $o$ to $o'$, whereas the number of matching pairs is not important for the decision. This observation inspires us to merge the matching objects into the same cluster, and then add the ``non-matching" labeled edges among different clusters. We call such graph as \clustergraph. By using the \clustergraph, we can efficiently decide whether a new pair $p=(o, o')$ can be deduced from the already labeled pairs. Figure~\ref{algo:deduce-label} shows the pseudo-code of the algorithm. Given a set of labeled pairs $\labelset$, we first build a \clustergraph for $\labelset$ (Line~\ref{algo:deduce-label:buildgraph}). Then for the unlabeled pair $p=(o, o')$, (1) if $o$ and $o'$ in the same cluster, then there is a path from $o$ to $o'$ which only consists of matching pairs, thus $o$ and $o'$ can be deduced as a matching pair (Lines~\ref{algo:deduce-label:matching-begin}-\ref{algo:deduce-label:matching-end}); (2)if $o$ and $o'$ in different clusters but there is an edge between them, then there exists a path from $o$ to $o'$ which contains a single non-matching pair, thus $o$ and $o'$ can be deduced as a non-matching pair (Lines~\ref{algo:deduce-label:nonmatching-begin}-\ref{algo:deduce-label:nonmatching-end}); If $o$ and $o'$ in different clusters and there is no edge between them, then there does not exist a path from $o$ to $o'$ which contains no more than one non-matching pair, thus $o$ and $o'$ cannot be deduced (Lines~\ref{algo:deduce-label:undeduced-begin}-\ref{algo:deduce-label:undeduced-end}).

\begin{figure}[htbp]
\centering
  \includegraphics[scale=0.35]{figs/cluster-graph.eps}\\
  \caption{A {$\clustergraph$} built for the first seven labeled pairs $\{p_1, p_2, \cdots, p_7\}$ in Figure~\ref{fig:framework}.}\label{fig:cluster-graph}
\end{figure}


\begin{example}
Suppose we have already labeled the first seven pairs $\{ p_1, p_2, \cdots, p_7\}$ in Figure~\ref{fig:deduce-graph}. To decide whether $p_8$ can be deduced from the already labeled pairs, we build a $\clustergraph$ as shown in Figure~\ref{fig:cluster-graph}. As $o_1, o_2, o_3$ are matching, we merge them into one cluster. As $o_4$ and $o_5$ are matching, we merge them into another cluster. Since $o_6$ does not match with any other object, we take itself as one cluster. After clustering all the matching objects in the $\clustergraph$, we obtain three clusters. In the already labeled pairs $\{ p_1, p_2, \cdots, p_7\}$, there are three non-matching pairs, i.e., $p_3=(o_1, o_6)$, $p_6=(o_4, o_6)$, $p_7=(o_2, o_4)$. We respectively add three non-matching edges between $\cluster{o_1}$ and $\cluster{o_6}$, $\cluster{o_4}$ and $\cluster{o_6}$, $\cluster{o_2}$ and $\cluster{o_4}$ to the $\clustergraph$.  For the unlabeled pair $p_8=(o_5, o_6)$, since $o_5$ and $o_6$ are in different clusters, and $\cluster{o_5}$ and $\cluster{o_6}$ have an edge in the \clustergraph, then there must exist a path from $o_5$ to $o_7$ which contains a single non-matching pair (i.e., $o_5\!\rightarrow\!o_4\!\rightarrow\!o_6$), thus $p_8=(o_5, o_6)$ can be deduced as a non-matching pair from the already labeled pairs $\{p_1, p_2, \cdots, p_7\}$.
\end{example}

%can be deduced as a matching pair since they are in the same cluster, and $(o_5, o_7)$ can be deduced as a non-matching pair since they are in different clusters and $\cluster{o_5}$ and $\cluster{o_7}$ have an edge, and $(o_1,o_7)$ cannot be deduced since they are in different clusters and $\cluster{o_1}$ and $\cluster{o_7}$ have no edge.




\iffalse
To build \clustergraph, initially, each object itself is taken as a cluster, and there is no edge among the clusters. Let $\cluster{o}$ denote $o$'s cluster. When adding a new pair $(o, o')$ to the graph, we consider the following cases: (1) If $o$ and $o'$ are in the same cluster, i.e. $\cluster{o} = \cluster{o'}$, the graph will keep unchanged; (2) If $o$ and $o'$ are in the different clusters, i.e. $\cluster{o} \neq \cluster{o'}$, and $o$ and $o'$ are non-matching, we will add an edge (if not exists) labeled ``non-matching" between \cluster{o} and \cluster{o'} to the graph; (3) If $o$ and $o'$ are in the different clusters, i.e. $\cluster{o} \neq \cluster{o'}$, and $o$ and $o'$ are matching, we will merge the objects in $\cluster{o}$ and $\cluster{o'}$ into a new cluster, and for each cluster that originally has an edge with $\cluster{o}$ or $\cluster{o'}$, we remove the edge from the graph, and then add a new edge with the merged cluster. For example, suppose  . To build .


\fi





\subsubsection{Crowdsourcing the label of an object pair}\label{subsubsec:label-crowdsourcing}
If a pair's label cannot be deduced from the already labeled pairs, we will create a Human Intelligent Task (HIT) for the pair, and publish it to a crowdsourcing platform. Figure~\ref{fig:hit-example} shows an example HIT for a pair (``\textsf{iPad 2}", ``\textsf{iPad two}"). In the HIT, there is a pair of strings, ``\textsf{iPad 2}" and ``\textsf{iPad two}", and the workers are required either select ``YES" if they think ``\textsf{iPad 2}" and ``\textsf{iPad two}" are mathing, or select ``NO" if they think ``\textsf{iPad 2}" and ``\textsf{iPad two}" are not matching, and then they submit their answers by clicking the \textsf{SUBMIT} button. After the crowd workers complete the HIT, we output the crowdsourced label of the pair.

\begin{figure}[htbp]
\centering
  \includegraphics[scale=0.3]{figs/hit.eps}\\
  \caption{An example HIT for an object pair.}\label{fig:hit-example}
\end{figure}

%\input{crowdsource-label-algo}



\subsection{Illustration of Hybrid Labeling framework}\label{subsec:workflow-example}

Typically, in a crowdsourcing platform, we need to pay for crowdsourced pairs, thus there is a financial incentive to minimize the number of crowdsourced pairs. Based on this idea, we propose a labeling framework as shown in  Figure~\ref{fig:framework}. Specifically, the framework consists of two steps.

%which will first seek to identify the best labeling order which results in the fewest number of crowdsourced pairs, and then label the object pairs in the identified order through crowdsourcing and transitive relation. Figure~\ref{fig:framework} shows our labeling framework.

\vspace{.5em}

{\noindent \bf Sorting}: At the first step, the framework takes as input a set of unlabeled pairs, and then identifies the best labeling order which could result in the fewest number of crowdsourced pairs, and finally outputs a sorted list of unlabeled pairs based on the order.

\vspace{.5em}

{\noindent \bf Labeling}: At the second step, the framework labels the pairs in the identified order through crowdsourcing and transitive relation. It utilizes the already labeled pairs to decide whether a new pair needs to be crowdsourced or can be deduced. If the label of the pair can be deduced from the already labeled pairs, the framework will output its deduced label; otherwise, the framework will publish the pair to the crowdsourcing platform, and output its crowdsourced label.








